TASM: A Tile-Based Storage Manager for Video Analytics

Modern video data management systems store videos as a single encoded file, which significantly limits possible storage level optimizations. We design, implement, and evaluate TASM, a new tile-based storage manager for video data. TASM uses a feature in modern video codecs called "tiles" that enables spatial random access into encoded videos. TASM physically tunes stored videos by optimizing their tile layouts given the video content and a query workload. Additionally, TASM dynamically tunes that layout in response to changes in the query workload or if the query workload and video contents are incrementally discovered. Finally, TASM also produces efficient initial tile layouts for newly ingested videos. We demonstrate that TASM can speed up subframe selection queries by an average of over 50% and up to 94%. TASM can also improve the throughput of the full scan phase of object detection queries by up to 2X.

==> icde_response.tex <==
%!TEX root = paper.tex

\section*{Response}

% \todo{In revising your paper, please go through the reviewer comments carefully, and substantively deal with the revision items raised by them. The main issues to be addressed are highlighted in the meta­-review.  Please provide a 3-page cover letter in the same PDF as your revision document, which lists the revision points and how and where in the draft they are addressed. Please make sure to highlight all modifications in the draft with a different color from the original text. This will help reviewers track and assess your changes. }

We thank the reviewers for their helpful comments and feedback! We addressed all of the comments, as we describe below. Changes to the original text are highlighted in blue.

\subsection*{Review responses}

\textbf{R1W1} 
ArrayStore (developed as part of the SciDB project) was a system designed for a different type of data: scientific arrays. Unlike video data, these arrays are high-dimensional, 
% \brandon{high-dimensional?  Video is also multidimensional (specifically 3D)}, 
each cell contains a tuple of values, and arrays are not expensive to encode or decode. The focus of ArrayStore was to identify techniques for breaking these large, multidimensional arrays into smaller chunks to make it efficient to process them in parallel, avoid skew, and join multiple arrays together. In prior work \cite{LightDB:pvldb/HaynesMABCC18}, we found that SciDB was not competitive for video data. Video data needs an entirely different design.

\textbf{R1W2} 
We added examples in \cref{sec:introduction} of applications that can benefit from the ability to operate over regions rather than full frames. Those
applications typically need to process or modify only a subset of a frame to compute a desired result. Another example application is the macro-benchmark query that
we added in response to the next comment (R1W3).


\textbf{R1W3} 
This is a good point. Our initial evaluation lacked an end-to-end application. We added an evaluation over a macro-benchmark query from the Visual Road benchmark to \cref{sec:macrobenchmarkEval}. This query detects objects (if they have not been detected yet), draws boxes around a specified object class, and returns the modified \textit{full} video frames. We demonstrate that TASM provides benefits despite the query returning full frames because only the subset of the frame that contains objects must be modified to add the bounding boxes, so TASM can decode and process fewer pixels. The full frames returned via homomorphic stitching (i.e., without decoding untouched tiles) have high quality, as we show in a sample frame from one of the 4K videos.

\begin{figure}[h]
\includegraphics[width=0.95\textwidth]{figures/revision/stitched_frame.jpg}
\end{figure}

\textbf{R1D1} 
See R1W3.

\textbf{R1D2} 
The median and IQR bars in the graphs show the performance \textit{across} videos. The bars can be quite large because different videos have different object densities, which affects TASM's performance as described in \cref{subsec:evalNonUniform}.
However, the runtime for a single query on any video has low variance. The standard deviation for multiple executions of the same query is $<1\%$ of that query's mean execution time.
We added this explanation to the evaluation in \cref{sec:evaluation}, just above the heading for \cref{sec:evaluation}(A).

\textbf{R1D3} 
This is a good point; the description of the application was lost when we edited the introduction.
We added a description of a city planning application before walking through the example in \cref{sec:unknownWorkloadUnknownObjects}.

% \magda{The answer to R1D4 is too long, defensive, and rambling. We need to make it concise and focused on the positive. My attempt is below:}
\textbf{R1D4}
Using an initial tiling around regions of interest is an optional step that we show can accelerate even the first object
detection query. We envision that such an initial tiling would be performed on the edge device that captures and encodes the video, which would eliminate TASM's overhead.
% The cost of background segmentation with OpenCV varies depending on the video content. The water's movement in the canal video that we use
% in the experiment challenges the background segmenter and achieves a throughput of 20 fps. A different video from BlazeIt's dataset that shows an intersection (jackson-town-square) achieves a throughput of over 40 fps. 
Cameras today are capable of running lightweight predicates as video is captured~\cite{boschCameraTrainer}, and specialized background subtractor modules can run at over 20 FPS on low-end hardware~\cite{fastestBackgroundSubtraction}. For comparison, running background segmentation with OpenCV in our experiments achieved a throughput of 20-40 fps depending on the video content.


%This cost of background segmentation along with the cost of encoding the video with tiles require tens of preprocessing queries to amortize because preprocessing the frames is relatively inexpensive (as indicated by the relatively high throughput for the baselines in \cref{fig:preprocessingTput}).

%However, we believe it is feasible to push lightweight ROI detection and the initial tiling step to the camera that initially captures the video, and thus eliminate this startup cost.

%A camera could initially encode the video with tiles around these detections to eliminate any added overhead.

We added a discussion about these initial costs to \cref{sec:ROI}. Additionally, we modified the experiment in \cref{sec:objectDetectionEval} to only run background segmentation on the first frame of each GOP, which is a throughput that cameras are known to operate at or above. Therefore, it would be possible for a camera at the edge to generate these detections in real time.
We used this limited set of detections to pick a tile layout for each GOP.
We also switched to use OpenCV's MOG2 background segmentation algorithm because it handled the water in the video better than the KNN-based algorithm.

We find that using the tile layouts designed after running background segmentation at a reduced frame rate led to similar improvements in preprocessing throughput. The model accuracy is a few points lower than when we used the tile layouts generated after running background segmentation on each frame, but it is still similar to the accuracy achieved when training the model with the full frames.


\textbf{R2W1} 
It is true that the specific performance will depend on the video and workload because the effectiveness of tiling depends on the density of the objects that are queried.
For an individual query, the maximum expected improvement is inversely proportional to the query object's density, which determines the number of pixels and tiles that must be processed.
TASM's techniques will not improve the performance of queries for very dense objects that take up most of the frame.
We updated \cref{sec:notation} to describe how the query object's density affects the expected performance improvements.
We also updated \cref{fig:tilingCutoff} to show the density of the query object to highlight how non-uniform layouts benefit sparse objects more than dense objects.

In terms of the effectiveness of the regret-based optimization, we assume some stability in the workload. 
If the workload is stable and there is some repetition in the queries, TASM will converge to the layout that minimizes the cost summed over the queries in the workload.
However, if the workload is random or frequently changing, our approach will face the same challenges as any dynamic tuning approach. The performance will suffer because the system never learns any useful information from past queries.

% "For individual frames, xxx. We updated Section XX." (= what we have been discussing in earlier emails).  Then we can add "In terms of the regret-based optimization, if the workload is stable, the approach will converge to the layout that minimizes the cost averaged/summed across all queries in the workload. In the case of changing workloads, like any dynamic tuning approach, the performance will only be good if there is some repetition in the queries, otherwise the system never learns any useful information from past queries." (we would need to articulate it better). If we do that, the reviewer can come back to us and clarify what they have in mind and what they would like to see updated/added.


% However, if objects are sparse enough we expect from our cost function that it should be possible to create a tile layout that accelerates queries, and therefore the regret-based approach will eventually pick that layout.
% We added an explanation to \cref{sec:notation} that describes how the expected improvements based on the cost function for a video with specific properties aligns with our experimental observations.
% \maureen{I think this may still sound like conclusion-by-observation.}

\textbf{R2D1} 
We expect that limiting the number of tiles, and therefore tile boundaries, would be an effective way to maintain PSNR above a user-specified limit. We added this explanation to \cref{sec:nonUniformLayouts}.

\textbf{R2D2} 
While the accuracies across days are not very similar, the accuracies within a given day are fairly close.
% \brandon{Is there an obvious reason for this difference across days, e.g., day/night or something?  The reviewer hasn't seen the actual videos.}.
The accuracy for all approaches differs across days because while the video for each day has the same field of view, the class distribution is slightly different across the videos. For example, the video from the second day contains more frames with $\geq3$ boats than the other two.
It is possible that, in some cases, the models trained on the tiled frames performed better because the tiled region omitted parts of the frame that did not contain the objects of interest, so the model learned from only the informative part of the frame.

\textbf{R3W1} 
This is a good point. Our usage of the term ``content retrieval'' was confusing because we do not support similarity search over videos. We rephrased all such references to ``subframe selection'' because our $\textsc{Scan}$ function returns the pixels from a subset of the frame. We also added a table to \cref{sec:api} to make it more clear what functions belong to the API, and what their return types are.

\textbf{R3W2} 
We added a brief discussion of tiles to the introduction. We also moved \cref{fig:tileAndFiles} to the introduction to illustrate how frames can be divided into tiles and that each tile contains a subset of the original frame.

\textbf{R3W3} 
We clarify in \cref{subsec:uniformtileseval} how the uniform tile configurations were chosen.
Briefly, we increased the number of uniform tiles first by increasing the number of rows and columns together, and then by only increasing the number of columns once the height of each tile reached the minimum height allowed by the decoder.

\textbf{R3D2} 
See R3W2.

\textbf{R3D3} 
See R3W1.

\textbf{R3D4} 
We added an explanation to \cref{sec:videoencoding} to clarify the relationship between tiles and frames. Both contain pixel information, however tiles only contain the pixels for a subset of the original frame.

\textbf{R3D5} 
See R3W3.

\textbf{R3D6} 
We added an explanation to \cref{sec:files} that describes how updates are handled. Because each video's data is stored separately, different videos are independent. Further, because each GOP within a video is also stored independently, to update a video, the system can update or add a GOP and the modified GOPs can replace the original ones.

\textbf{R3D7} 
While we use SQL to explain the experiments because of its familiarity to most readers, other language bindings on top of TASM's API are possible. The language itself is not the focus of this paper. We added this explanation to \cref{sec:evaluation}, where the queries are presented.

\subsection*{Other changes}
\textbf{Figure 12}
While implementing the new experiments, we noticed an extra optimization opportunity when tiling around all objects. The optimization is to add an index to the labels table using the search key (frame, label). This optimization had a minor impact on Figure 12, which we updated. All trends remain the same. The line showing the performance of tiling around all objects has slightly better numbers.


==> queries.tex <==
\section{Queries} 

\subsection{Queries from papers}
\begin{itemize}
    \item Amber alert: retrieve a vehicle of a certain color, type, and license plate number~\cite{DBLP:conf/cloud/LuCK16}
    \begin{itemize}
        \item Multi-query scenario: The first query is for color + type + license plate number. Suppose it doesn't return much because maybe license plate recognition failed on some cameras. The user issues a second query for just color + type.
    \end{itemize}
    \item Traffic violation: detect vehicles that are speeding, weaving between lanes, or making illegal turns~\cite{DBLP:conf/cloud/LuCK16}
    \begin{itemize}
        \item Multi-query scenario: Issue them as three separate queries. It seems likely that at least some of the speeding cars were also weaving between lanes.
    \end{itemize}
    \item Re-identification: retrieve a vehicle of the same type across two different cameras~\cite{DBLP:conf/cloud/LuCK16}
    \begin{itemize}
        \item Multi-query scenario: Maybe the same query is issued multiple times for different vehicle types.
    \end{itemize}
    \item License plate reader: OpenALPR library scans the video frame to detect potential plates~\cite{VideoStorm:nsdi/ZhangABPBF17}
    \begin{itemize}
        \item Multi-query scenario: Maybe the first query is for the exact license plate match. Maybe not as many results are returned, so future queries include similar license plate numbers.
    \end{itemize}
    \item Car counter: monitor areas of interest and count cars passing the area~\cite{VideoStorm:nsdi/ZhangABPBF17}
    \begin{itemize}
        \item Multi-query scenario: Maybe the area of interest changes between queries. One query could be interested in the HOV lane, and another query could be interested in the entrance ramp to the highway.
    \end{itemize}
    % \item DNN classifier: object recognition and classification~\cite{VideoStorm:nsdi/ZhangABPBF17}
    % \item Object tracker: track objects across frames~\cite{VideoStorm:nsdi/ZhangABPBF17}
    % \item Augmented reality: detect objects in live streaming video \& overlay the bounding boxes.~\cite{LightDB:pvldb/HaynesMABCC18}
    % \begin{itemize}
    %     \item Multi-query scenario: Maybe the objects of interest change between queries.
    % \end{itemize}
    % \item Find all frames that contain objects of class $X$~\cite{Focus:osdi/HsiehABVBPGM18}
    % \begin{itemize}
    %     \item Multi-query scenario: Maybe the class $X$ changes between queries.
    % \end{itemize}
    \item Object detection: identify objects of interests, their classes, and locations in each frame.~\cite{Chameleon:sigcomm/JiangABSS18}
    \begin{itemize}
        \item Multi-query scenario: Maybe the objects of interest change between queries.
    \end{itemize}
    \item Urban planning: Determine the busiest times. Find 10 events of at least 1 bus and 5 cars. Find red buses.~\cite{BlazeIt:corr/abs-1805-01046}
    \begin{itemize}
        \item Multi-query scenario: The idea of what constitutes "busy" changes between queries. For the first query it could be 1 bus and 5 cars, but the next could ask for 2 buses and 7 cars.
    \end{itemize}
    \item Autonomous vehicle analysis: Find events where there is a yellow light and multiple pedestrians in the crosswalk.~\cite{BlazeIt:corr/abs-1805-01046}
    \item Store planning: Count the number of people who walk through each aisle~\cite{BlazeIt:corr/abs-1805-01046}
    \begin{itemize}
        \item Multi-query scenario: First the owner wants to see people in aisle 1, then aisle 5.
    \end{itemize}
    \item Ornithology: Count the number of birds that visit each side of a bird feeder. Select red or blue birds.~\cite{BlazeIt:corr/abs-1805-01046}
    \begin{itemize}
        \item Multi-query scenario: As described in the original example, people may want to see birds of different colors.
    \end{itemize}
    % \item Large-scale video data mining: object tracking, object detection, activity recognition, frame segmentation~\cite{Scanner:tog/PomsCHF18}
    \item Find clips of interviews of Bernie Sanders by Jake Tapper.~\cite{Rekall:corr/abs-1910-02993}
    \begin{itemize}
        \item Multi-query scenario: Maybe the people change between the queries. As described in the paper, the query proceeds in multiple steps (find faces, find Bernie Sanders's face, find Jake Tapper's face, find clips where Bernie appears before or after Jake). The execution of the query wouldn't have to go through all of these separate steps, but if a user were trying to debug a query they may execute each of these steps separately.
    \end{itemize}
    \item Did Donald Trump or Hillary Clinton get more interview screen time in the months before the 2016 election?~\cite{Rekall:corr/abs-1910-02993}
    \item How much more screen time is given to male presenting vs. female presenting hosts?~\cite{Rekall:corr/abs-1910-02993}
    \item Find traffic light changes in quick succession~\cite{Rekall:corr/abs-1910-02993}
    \begin{itemize}
        \item Multi-query scenario: Maybe the definition of ``quick'' changes between queries, or the second query focuses on one particular intersection.
    \end{itemize}
    \item Find turns by other vehicles near the autonomous vehicle~\cite{Rekall:corr/abs-1910-02993}
    \item Find frames with at least two woman faces~\cite{Rekall:corr/abs-1910-02993}
    \item Generic querying tasks from Panorama~\cite{Panorama:pvldb/ZhangK19}
    \begin{itemize}
        \item Recognition: Identify objects present in a given frame
        \item Localization: Identify the regions of a frame where objects exist
        \item Verification: Identify if the same object occurs in both frames
    \end{itemize}
    \item What are the license plate numbers of all blue cars in the last week?~\cite{VStore:eurosys/XuBL19}
    \item Find cars~\cite{VStore:eurosys/XuBL19}
    % \item Run license plate recognition~\cite{VStore:eurosys/XuBL19}
    \item Find all videos of automobiles exceeding $n$ kilometers per hour~\cite{VisualWorldDB:cidr/HaynesDMBCC20}
    \item How many automobiles transited an intersection per hour?~\cite{VisualWorldDB:cidr/HaynesDMBCC20}
\end{itemize}

\subsection{Other query ideas}
\begin{itemize}
    \item Drone videos for animal conservation. Some queries may be for specific animals to check their wellbeing, and other queries may be for humans to find potential poachers.
    \item Traffic videos.
    \begin{itemize}
        \item Civil engineers may be interested in counting the number of cars.
        \item Police may be interested in finding cars with specific license plates, cyclists without helmets, or HOV lane violators.
        \item Government officials may be interested in finding potholes.
        \item Researcher may be interested in building a diverse training set for a ML model and ask for instances of different car types.
    \end{itemize}
    \item Home surveillance
    \begin{itemize}
        \item Find all of the dogs. Then find all of the people. Then find all of the people walking with dogs.
    \end{itemize}
    \item Recent work uses compositional event specification to detect novel events in video~\cite{Rekall:corr/abs-1910-02993}. This is a repetitive process as users figure out the correct composition for the events they are interested in. As users navigate this repetitive process, there will be many similar queries over the video.
\end{itemize}

\subsection{General patterns in queries}
\begin{itemize}
    \item Queries get more and more broad, so results of future queries include the results of previous queries plus some. (e.g. search for blue Toyota with a particular license plate, then search for just blue Toyotas)
    \item Queries get more and more narrow, so results of future queries are a subset of the results of previous queries. (e.g. search for blue Toyotas, then search for blue Toyotas with a particular license plate at a particular intersection)
    \item Changing queries. Results from future queries may or may not overlap with results from previous queries. (e.g. first search for object of type A, then type B)
\end{itemize}

